DDES Study of Confined and Unconfined NACA Wing Sections Using Spectral Elements

We develop hybrid RANS-LES strategies within the spectral element code Nek5000 based on the $k-\tau$ class of turbulence models. We chose airfoil sections at small flight configurations as our target problem to comprehensively test the solver accuracy and performance. We present verification and validation results of an unconfined NACA0012 wing section in a pure RANS and in a hybrid RANS-LES setup for an angle of attack ranging from 0 to 90 degrees. The RANS results shows good corroboration with existing experimental and numerical datasets for low incoming flow angles. A small discrepancy appears at higher angle in comparison with the experiments, which is in line with our expectations from a RANS formulation. On the other hand, DDES captures both the attached and separated flow dynamics well when compared with available numerical datasets. We demonstrate that for the hybrid turbulence modeling approach a high-order spectral element discretization converges faster (i.e., with less resolution) and captures the flow dynamics more accurately than representative low-order finite-volume and finite-difference approaches. We also revise some of the guidelines on sample size requirements for statistics convergence. Furthermore, we analyze some of the observed discrepancies of our unconfined DDES at higher angles with the experiments by evaluating the side wall "blocking" effect. We carry out additional simulations in a confined 'numerical wind tunnel' and assess the observed differences as a function of Reynolds number.

==> tex/backmatter.tex <==

\begin{Backmatter}

\paragraph{Acknowledgements}
We gratefully acknowledge the help of Yuhsiang Lan who
provided technical support during the simulations.

\paragraph{Funding Statement}
%J.G.S gratefully acknowledges funding by an NSF CAREER
%Award (Contract number NSF CTS0239080) with Dr. Michael W.
%Plesniak as contract monitor.

\paragraph{Declaration of Interests}
The authors declare no conflict of interest.

\paragraph{Author Contributions}
M.M. and P.F. created the research plan, A.T. implemented
the numerical tools. V.K. performed the simulations and wrote 
the first draft of manuscript. All authors contributed in revisions.

\paragraph{Data Availability Statement}
Raw data are available from the corresponding author
(V.K.).

\paragraph{Ethical Standards}
The research meets all ethical guidelines, including
adherence to the legal requirements of the study country.

\paragraph{Supplementary Material}
%Methods section and Supplementary information are available
%at \url{https://doi.org/10.1017/flo.2021.1}.


%\begin{thebibliography}{}
% \input tex/biblist 
%\end{thebibliography}
\bibliographystyle{plainnat}
\bibliography{bibs/emmd,bibs/ananias,bibs/abl,bibs/references.bib,bibs/vishal.bib}

\end{Backmatter}

\end{document}


==> tex/biblist.tex <==
\bibitem[Piomelli (2014)]{Piomelli2014}
Piomelli, U. (2014). Large eddy simulations in 2030 and beyond.
\textit{Philos Trans R Soc A Math Phys Eng Sci}. 372(2022):20130320

\bibitem[Choi \& Moin (2012)]{Choi2012}
Choi H, Moin P. (2012). Grid-point requirements for large eddy 
simulation: Chapman's estimates revisited. 
\textit{Phys Fluids}. 24(1):011702


==> tex/impact.tex <==


\begin{boxtext}

\textbf{\mathversion{bold}Impact Statement}

High Reynolds number aerodynamic predictions rely on the accuracy of low-fidelity 
turbulence closures.  It is often touted that high order methods do not necessarily
provide any advantage, over their low-order counterparts, for low fidelity turbulence
closures.  We provide evidence that argument doesnot hold true for missively separated 
aerodynamic flows.
 
\end{boxtext}


